ScoreNet: Learning Non-Uniform Attention and Augmentation for Transformer-Based Histopathological Image Classification

Progress in digital pathology is hindered by high-resolution images and the prohibitive cost of exhaustive localized annotations. The commonly used paradigm to categorize pathology images is patch-based processing, which often incorporates multiple instance learning (MIL) to aggregate local patch-level representations yielding image-level prediction. Nonetheless, diagnostically relevant regions may only take a small fraction of the whole tissue, and current MIL-based approaches often process images uniformly, discarding the inter-patches interactions. To alleviate these issues, we propose ScoreNet, a new efficient transformer that exploits a differentiable recommendation stage to extract discriminative image regions and dedicate computational resources accordingly. The proposed transformer leverages the local and global attention of a few dynamically recommended high-resolution regions at an efficient computational cost. We further introduce a novel mixing data-augmentation, namely ScoreMix, by leveraging the image's semantic distribution to guide the data mixing and produce coherent sample-label pairs. ScoreMix is embarrassingly simple and mitigates the pitfalls of previous augmentations, which assume a uniform semantic distribution and risk mislabeling the samples. Thorough experiments and ablation studies on three breast cancer histology datasets of Haematoxylin & Eosin (H&E) have validated the superiority of our approach over prior arts, including transformer-based models on tumour regions-of-interest (TRoIs) classification. ScoreNet equipped with proposed ScoreMix augmentation demonstrates better generalization capabilities and achieves new state-of-the-art (SOTA) results with only 50% of the data compared to other mixing augmentation variants. Finally, ScoreNet yields high efficacy and outperforms SOTA efficient transformers, namely TransPath and SwinTransformer.

==> experiments.tex <==
\section{Experiments}
\label{sec:experiments}
\vspace{1ex} \noindent \textbf{Datasets.}
The primary dataset used in our experiments is the BReAst Carcinoma Sub-typing (\textbf{BRACS})~\cite{PATI2022102264}. BRACS consists of $4391$ RoIs acquired from $325$ $\he$ stained breast carcinoma $\wsi$ (at $0.25$ $\mu$m/pixel) with varying dimensions and appearances. Each RoI is annotated with one of the seven classes: Normal, Benign, Usual Ductal Hyperplasia (UDH), Atypical Ductal Hyperplasia (ADH), Flat Epithelial Atypia (FEA), Ductal Carcinoma In Situ (DCIS), and Invasive. Our experiments follow the same data splitting scheme as \cite{PATI2022102264} for training, validation, and test set at the $\wsi$ level to avoid test leakage. In addition, we use publicly available BreAst Cancer Histology \textbf{(BACH)} dataset~\cite{ARESTA2019122} to show $\scorenet$ generalization capabilities. It contains $400$ training and $100$ test images from four different breast cancer types: Normal,  Benign, In Situ, and Invasive. All images have a fixed size of $1536 \times 2048$ pixels and a pixel scale of $0.42 \times 0.42$ $\mu$m. To assess the interpretability of $\scorenet$, we further evaluate our model on the \textbf{CAMELYON16} dataset~\cite{camelyon16} for binary tumour classification. We extract a class-balanced dataset of $1920\times1920$ pixels from high-resolution $\wsi$s.

\input{tables/trois_f1_scores}

\vspace{1ex} \noindent \textbf{Experimental Setup.}
\label{sec:experimentalsetting}
We base $\scorenet$' ViTs, namely the one used by the recommendation stage and by the local fine-grained attention mechanism on a modified ViT-tiny architecture (see \textbf{Supplementary Material}) and follow the self-supervised pre-training scheme of \cite{caron2021emerging} for both of the aforementioned $\vit$s. Noteworthy that an end-to-end pre-training of $\scorenet$ is also feasible.
After pre-training, the $\scorenet$ is optimized using the SGD optimizer (momentum=0.9) with a learning rate chosen with the linear scaling rule \cite{goyal2018accurate} ($lr=10^{-2}\cdot \text{batchsize} / 256 = 3.125\cdot10^{-4}$) annealed with a cosine schedule until $10^{-6}$. $\scorenet$ is finetuned for $15$ epochs with a batch-size of $8$. We empirically determine the top $K=20$ regions, and a downscaling factor $s=8$ by a hyperparameter sweep (cf. ablation experiment in the \textbf{Supplementary Material}).
All experiments are implemented in PyTorch 1.9 \cite{paszke2019pytorch} using a single GeForce RTX3070 GPU.

\subsection{TRoIs Classification Results and Discussion}
\label{subsubsec:trois_classification}
In Table~\ref{table:f1_scores_trois}, we compare the $\trois$ classification performance of $\scorenet$ on the BRACS dataset against the state-of-the-arts, including MIL-based~\cite{mercan2019patch,shao2021transmil,lu2021data}, GNN-based, e.g.,~\cite{PATI2022102264}, and self-supervised transformer-based~\cite{wang2021transpath} approaches. The first $\mil$-based baseline~\cite{mercan2019patch} aggregates independent patch representations from the penultimate layer of a ResNet-50 \cite{he2016deep} pre-trained on ImageNet \cite{5206848}. The patch model is further finetuned on $128\times128$ patches at different magnification, e.g., $10\times$, $20\times$ or $40\times$. The latter operate either on multi- or single-scale images to benefit from varying levels of context and resolution. Similarly, we report the performances of the recent MIL-based methods, TransMIL \cite{shao2021transmil}, and CLAM \cite{lu2021data} using the original implementations and setup. Both methods are tested with different magnifications (see Table \ref{table:f1_scores_trois}). Additionally, the single-head (-SB) and multi-head (-MB) variants of CLAM are used with the small (-S) and big (-B) versions of the models (see CLAM's implementation). We further use various GNN-based baselines, particularly HACT-Net \cite{PATI2022102264}, the current SOTA approach for $\troi$ classification on the BRACS. Finally, we report the performance of the recent self-supervised transformer approach, TransPath \cite{wang2021transpath}, which is a hybrid transformer/convolution-based architecture. $\scorenet$ reaches a new state-of-the-art weighted F1-score of $64.4\%$ on the BRACS $\troi$ classification task outperforming the second-best method, HACT-Net, by a margin of $2.9\%$ (Table \ref{table:f1_scores_trois}). The results are reported for two variants of  $\scorenet$, namely $\mathrm{ScoreNet/4/1}$ and $\mathrm{ScoreNet/4/3}$, which use the four last \texttt{[CLS]} tokens of the scorer and the last or the three last \texttt{[CLS]} tokens from the coarse attention mechanism (aggregation stage). $\mathrm{ScoreNet/4/3}$ variant puts more emphasis on the features available at (40$\times$), whereas $\mathrm{ScoreNet/4/1}$ is more biased towards the global representation available at (5$\times$) (with a downscaling factor $s=8$). One can observe that both model variants significantly outperform the existing baseline in terms of weighted F1-scores and for almost every class. More interestingly, the architectural differences directly translate to differences in the classification results. $\mathrm{ScoreNet/4/3}$ is more suitable for classes where the \textbf{discriminative features are at the cell level than $\mathrm{ScoreNet/4/1}$, which is more suited when the tissue organization is the discriminative criterion}. Nonetheless, both of these architectures indeed benefit from the information available at each scale. This observation is well supported by the classification results obtained when a linear layer is trained independently on the scorer's \texttt{[CLS]} tokens (Lin. scorer's \texttt{[CLS]} in Table \ref{table:f1_scores_trois}) or using only the \texttt{[CLS]} tokens from the aggregation stage (Lin. encoder's \texttt{[CLS]} in Table \ref{table:f1_scores_trois}). Despite the difference in results between the two model variants, it is clear that they both perform worse when separated, which indicates that the representations of both stages are complementary. In brief, $\scorenet$ allows for an easily tuning to meet prior inductive biases on the ideal scale for a given task.


\vspace{1ex} \noindent \textbf{ScoreMix \& Data-Regime Sensitivity.}
\label{par:scoremix_results}
We also show that $\scorenet$ equipped with the proposed $\scoremix$ augmentation achieves superior TRoIs classification performances compared to CutMix \cite{yun2019cutmix} and SaliencyMix \cite{uddin2020saliencymix} augmentations for different data regimes, e.g., low-regime with only $10\%$ of the data. \textbf{Our proposed $\score$ outperforms SOTA methods with only 50\% of the data} and is on-par or better than most baselines with only $20\%$ of the data (Table \ref{table:augmentation_comp}). We argue that these improvements are primarily due to the generation of more coherent sample-label pairs under the guidance of the learned semantic distribution. This alleviates randomly cutting and pasting non-discriminative patches, as is the case with CutMix. Our results further support that image saliency used in the SaliencyMix is not correlated with discriminative regions.

\input{tables/augmentation_comparison}
\vspace{1ex} \noindent \textbf{Generalization Capabilities.}
\label{subsubsec:generalization_camelyon}
To gauge the generalization capabilities of $\scorenet$ compared to other current SOTA methods, e.g., HACT-Net~\cite{pati2020hact}, we leverage two external evaluation datasets, namely CAMELYON16 and BACH. After training on the BRACS dataset, the weights of $\scorenet$ are frozen. To evaluate the quality of the learned features, we either train a linear classifier on top of the frozen features or apply a $k$-nearest-neighbor classifier ($k$ = 1) without any finetuning. We perform stratified 5-fold cross-validation. For HACT-Net, we use the available pre-trained weights and follow the implementation of~\cite{PATI2022102264}. As HACT-Net sometimes fails to generate embeddings and to have a fair comparison, we only evaluate the samples for which HACT-Net could successfully produce embeddings (around $95\%$ of the BACH and $80\%$ of the CAMELYON16 datasets). Experimental results in Table~\ref{tab:generalization} demonstrate the superiority of $\scorenet$ in learning generalizable features. It further demonstrates the robustness of $\scorenet$ to changes in magnification. Indeed, the model is pre-trained on BRACS (40$\times$), while BACH’s images were acquired at a magnification of 20$\times$. Furthermore, the CAMELYON16 dataset contains $\wsis$ collected from lymph nodes in the vicinity of the breast, while BRACS contains $\wsis$ collected by mastectomy or biopsy (i.e., directly in the breast). The excellent knowledge transfer between the two datasets highlights the transferability of features learned by $\scorenet$ in various use cases.
\input{tables/generalization_capabilities}
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{figures/interpretability.png}
    \caption{\textbf{$\snet$ Interpretability}. Visualization of the semantic distribution, overlaid with the tumour ground-truth mask on a few samples of the CAMELYON16 dataset. The semantic distributions are obtained from the recommendation stage, i.e., at low-resolution. $\scorenet$ is pre-trained on BRACS and finetuned on CAMELYON16.}
    \label{fig:interpretability}
\end{figure} 

\vspace{1ex} \noindent \textbf{Interpretability?}
\label{subsubsec:interpretability}
To probe the internal behavior of $\scorenet$, we finetune the model on CAMELYON16 images using image-level labels only. At test time, we scrutinize the learned semantic distributions of the tumour-positive images. The semantic distributions depicted in Fig.~\ref{fig:interpretability} seems to indicate that $\scorenet$ learns to identify the tumour area and interpret \textbf{cancer-related morphological information}, while never having been taught to do so.
Quantitatively, we observe that, on average, $74.6 \%$ of the $20$ patches selected from positive images are tumour-positive. Furthermore, we report an average image-wise AuC of 73.6\% when interpreting the probability of the recommendation stage to sample a patch as the probability of it being tumour-positive. 

 \vspace{1ex} \noindent \textbf{Ablation on Efficacy of $\snet$.}
 \label{subsubsec:efficiency}
 The critical aspect of $\scorenet$ is its improved efficiency compared to other transformer-based architectures. This improvement is due to the choice of a hierarchical architecture and the exploitation of redundancy in histology images. At inference time, we expect a gain in throughput compared to the vanilla $\vit$ of the order of the squared downscaling factor, $s$, (see \textbf{Supplementary Material}), typically $s^2 = 64$, which is well reflected in practice, as shown in Table~\ref{table:throughput}. Due to the self-supervised pre-training, $\scorenet$ does not require any stain normalization or pre-processing, unlike its competitor HACT-Net. Similarly, ScoreNet yields higher throughput than other SOTA efficient transformers architectures, namely TransPath \cite{wang2021transpath}, and SwinTransformer \cite{liu2021swin}, with throughput around $3\times$ and $4\times$ higher than these methods. The latter observation is interesting considering the linear asymptotic time and memory cost of the SwinTransformer, which is probably a consequence of the fact that SwinTransformers process a lot of uninformative high-resolution patches in the first layer(s). 
 
\input{tables/throughput} 
\vspace{1ex} \noindent \textbf{Ablation on Shape Cues and Robustness.}
\label{par:shape_cues}
We investigate $\scorenet$’s ability to learn shape-related features. To do so, we study shape cues extracted by the recommendation model via the concatenated \texttt{[CLS]} tokens (see Fig.~\ref{fig:troi_architecture}). Consequently, we implement shape removal by applying a random permutation of the downscaled image’s tokens at test time. With this setup, a weighted F1-score of 59.8 $\pm$ 0.8\% is reached, representing a significant drop in performance compared to 64.4 $\pm$ 0.9\% without permutation. It demonstrates that \textit{i)} the recommendation stage's concatenated \texttt{[CLS]} tokens contribute positively to the overall representation and \textit{ii)} the latter is \textbf{not permutation invariant} and thus shape-dependent.  In a second experiment, we show the whole recommendation stage is also shape-dependent. To that end, we repeat the same experiment, but the patches are extracted from the permuted images, reaching a weighted F1-score of 59.5 $\pm$ 0.6\%. We further observe that for a given image, the overlap of the selected patches with and without permutation is, on average, only $15.7\%$, which indicates that the semantic distribution learned by $\scorenet$ is shape-dependent. 


==> methods.tex <==
\section{Methods}
\label{sec:methodo}
\vspace{1ex} \noindent \textbf{Model Overview.} \label{subsec:method:TRoIs_model} An overview of the proposed training pipeline for $\he$ stained histology $\trois$' representation learning is illustrated in Fig.~\ref{fig:troi_architecture}. Histopathological image classification requires capturing cellular and tissue-level microenvironments and learning their respective interactions. Motivated by the above, we propose an efficient transformer, $\scorenet$ that captures the cell-level structure and tissue-level context at the most appropriate resolutions. Provided sufficient contextual information, we postulate and empirically verify that a tissue's identification can be achieved by only attending to its sub-region in a high-resolution image. As a consequence, $\scorenet$ encompasses two stages. The former (\textit{differentiable recommendation}) provides contextual information and selects the most informative high-resolution regions. The latter (\textit{aggregation and prediction}) processes the recommended regions and the global information to identify the tissue and model their interactions simultaneously.

More precisely, the recommendation stage is implemented by a $\vit$ and takes as input a downscaled image to produce a semantic distribution over the high-resolution patches. Then, the most discriminative high-resolution patches for the end task are \textbf{differentiably extracted}. These selected patches (tokens) are then fed to a second $\vit$ implementing the \textit{local fine-grained attention} module, which identifies the tissues represented in each patch. Subsequently, the \textbf{embedded patches attend to one another via a transformer encoder} (\textit{global coarse grained  attention}). This step concurrently refines the tissues' representations and model their interactions. As a final step, the concatenation of the \texttt{[CLS]} tokens from the recommendation's stage and that of the \textit{global coarse-grained attention}'s encoder produces the image's representation. Not only does $\scorenet$'s workflow allows for a significantly increased throughput compared to SOTA methods (see Table~\ref{table:throughput}), it further enables the independent pre-training and validation of its constituent parts.

\subsection{ScoreNet}
\label{subsec:method:scorenet}
\vspace{1ex} \noindent \textbf{Semantic Regions Recommendation.}
\label{subsubsec:patch_selection}
Current $\mil$-based approaches~\cite{ilse2018attention,li2021dual} based on patch-level features aggregation often process histopathological images uniformly and discard the inter-patches interactions. To alleviate these issues, we exploit \textbf{a differentiable recommendation stage to extract discriminative image regions relevant to the classification}. More specifically, we leverage the self-attention map of a $\vit$ as a distribution of the semantic content. Towards that end, the high-resolution image is first downscaled by a factor $s$ and subsequently fed to the recommendation's stage $\vit$. The resulting self-attention map captures the contribution of each patch to the overall representation. Let's assume a $\vit$, that processes a low-resolution image $x_{l} \in \mathbb{R}^{C \times h \times w}$ encompassing $N$ patches of dimension $P_{l} \times P_{l}$. The attended patches (tokens) of the $(L-1)$ layer are conveniently represented as a matrix $\textbf{Z} \in \mathbb{R}^{\left(N+1\right) \times d}$, where $d$ is the embedding dimension of the model, and the extra index is due to the \texttt{[CLS]} token. Up to the last MLP and for a single attention head, the representation of the complete image is given by:
\begin{equation}
\label{eq:y_cls}
    y_{[\text{CLS}]} = \underbrace{\text{softmax}(a_{1}^{T})}_{1 \times (N+1)}\underbrace{\textbf{ZW}_{\text{val}}}_{(N+1) \times d}
    % y_{[\text{CLS}]} = \text{softmax}(a_{1}^{T}) \textbf{XW}_{\text{val}}
\end{equation}
%
where $\textbf{W}_{\text{val}} \in \mathbb{R}^{d \times d}$ is the value matrix, and $a_{1}^{T}$ is the first row of the self-attention matrix \textbf{A}:
% $\textbf{A}= \textbf{XW}_{\text{qry}} \left( \textbf{XW}_{\text{key}}\right)^T \in \mathbb{R}^{(N+1) \times (N+1)}$.
\begin{equation}
    \textbf{A} = \textbf{ZW}_{\text{qry}} \left( \textbf{ZW}_{\text{key}}\right)^T
\end{equation}
%
where $\textbf{W}_{\text{qry}}$ and $\textbf{W}_{\text{key}}$ are the query and key matrices, respectively. The first row of the self-attention matrix captures the contribution of each token to the overall representation (Eq.~\ref{eq:y_cls}). This is in line with the discriminative capacity of the \texttt{[CLS]} token that patches having the highest contribution are the ones situated in the highest semantic regions of the images. The distribution of the semantic content over the patches is therefore defined as:
\begin{equation}
\label{eq:dist_patch}
    \mathbb{P}_{\text{patch}} = \text{Softmax}(\Tilde{a}_{1}^{T}) \in \mathbb{R}^{N}
\end{equation}
%
where $\Tilde{a}_{1}$ stands for $a_{1}$ without the first entry, namely the one corresponding to the \texttt{[CLS]} token. Since $\vit$s typically encompasses multiple heads, we propose to add an extra learnable parameter, which weights the relative contributions of each head to the end task; after aggregation of the multiples self-attention maps, the formulation is identical to that of Eq.~\ref{eq:dist_patch}.

Concurrently with acquiring the above defined semantic distribution, the high-resolution image, $x_{h} \in \mathbb{R}^{C \times H \times W}$, is tiled in a regular grid of large patches ($P_{h} \times P_{h}$), stored in a tensor $\textbf{P} \in \mathbb{R}^{N \times C \times P_{h} \times P_{h}}$. At inference time, a convenient way to select the $K$ most semantically relevant high-resolution regions is to encode the \textit{top-K} indices as one-hot vectors: $\textbf{Y} \in \mathbb{R}^{N \times K}$, and to extract the corresponding $K$ patches, $\textbf{X} \in \mathbb{R}^{K \times C \times P_{h} \times P_{h}}$ via: 
\begin{equation}
    \label{eq:patch_extraction}
    \textbf{X} = \textbf{Y}^{T} \textbf{P}
\end{equation}
%
At training time, since the above formulation is not differentiable, we propose to adopt the differentiable approach of~\cite{cordonnier2021differentiable}. Following the perturbed optimizers scheme, the \textit{top-K} operation is bootstrapped by applying a Gaussian noise, $\sigma \textbf{Z}$, to the semantic distribution. The noisy indicators, $\textbf{Y}_{\sigma}$, are subsequently computed as:
\begin{equation}
    \label{eq:topk_forward}
    \textbf{Y}_{\sigma} = \mathbb{E}_{\mathbf{Z}}\left[ \argmax_{\textbf{Y} \in \mathcal{C} } \left<\textbf{Y}, \Tilde{\mathbb{P}} + \sigma \textbf{Z} \right> \right]
\end{equation}
%
where $\sigma$ is the standard deviation of the noise, $\Tilde{\mathbb{P}} \in \mathbb{R}^{N \times K}$ is obtained by broadcasting $\mathbb{P}_{\text{patch}}$ to match the dimension of $\textbf{Y}$, and $\mathcal{C}$ is a restriction of the domain ensuring the equivalence between solving Eq.~\ref{eq:topk_forward} and the \textit{top-K} operation \cite{cordonnier2021differentiable}. The extraction of the high-resolution regions follows the procedure described in Eq.~\ref{eq:patch_extraction}. Similarly, the gradient of the indicators w.r.t. the semantic distribution, $\mathbb{P}_{\text{patch}}$ can be computed as:
\begin{equation}
    \label{eq:topk_backward}
        \nabla \textbf{Y}_{\sigma} = \mathbb{E}_{\mathbf{Z}}\left[ \argmax_{\textbf{Y} \in \mathcal{C} } \left<\textbf{Y}, \Tilde{\mathbb{P}} + \sigma \textbf{Z} \right> \textbf{Z}^{T} / \sigma \right]
\end{equation}

\vspace{1ex} \noindent \textbf{Computational Complexity.}
\label{subsubsec:comp_comp}
Vision transformers heavily rely on the attention mechanism to learn a high-level representation from low-level regions. The underlying assumption is that the different sub-regions of the image are not equally important for the overall representation. Despite this key observation, the computation cost dedicated to a sub-region is independent of its contribution to the high-level representation, which is inefficient. Our $\scorenet$ attention mechanism overcomes this drawback by learning to attribute more resources to regions of high interest. For a high-resolution input image $x_{h} \in \mathbb{R}^{C \times H \times W}$, the asymptotical time and memory cost is $\mathcal{O} \left(\left( \frac{H}{s \cdot P_{l}} \cdot \frac{W}{s \cdot P_{l}}\right)^2\right)$, when the recommendation stage uses inputs downscaled by a factor $s$ and processes them with a patch size of $P_{l}$. The derivation of this cost, including that of the recommendation stage, which is independent of the input size, can be found in the \textbf{Supplementary Material}.

\subsection{ScoreMix}
\label{subsec:method:score_mix}
We propose a new mixing data augmentation for histopathological images by learning the \textbf{distribution of the semantic image regions} using the learned self-attention for \texttt{[CLS]} token of the $\vit$ without requiring architectural changes or additional loss. 
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{bboxsampling.pdf}
    \caption{\textbf{The bounding box selection scheme for ScoreMix.} The score distribution for each bounding box ($\mathbb{P}_{\text{bbox}}$) is obtained by convolving the patch distribution map $\mathbb{P}_{\text{patch}}$ with a kernel of $\textbf{1}$s of the bounding box dimensions $(h_{\text{bbox}}, w_{\text{bbox}})$. The bbox is then sampled from $\mathbb{P}_{\text{bbox}}$, which we often refer to as $\mathbb{P}_{\text{source}}$ or $\mathbb{P}_{\text{target}}$.}
    \label{fig:bbox_sampling}
\end{figure}
More formally, let $x_{s}, x_{t} \in \mathbb{R}^{C \times H \times W}$ be the source and target images respectively and let $y_{s}$ and $y_{t}$ be their corresponding labels. We aim to mix the source and target samples to generate a new training example $(x_{m}, y_{m})$. To do so, we first compute the semantic distributions using the current parameters of the model and the input samples; namely, we compute $\mathbb{P}_{\text{source}}(x_{s}, \theta)$ and $\mathbb{P}_{\text{target}}(x_{t}, \theta)$. Given these distributions and a randomly defined bounding box size, we sample the cutting and pasting locations from the source and target distributions, respectively:
\begin{equation}
    \begin{aligned}
    M_{s} & \sim \frac{1}{Z_{s}} \cdot \mathbb{P}_{\text{source}}(x_{s}, \theta, \lambda) \\
    M_{t} & \sim \frac{1}{Z_{t}} \cdot \left(1 - \mathbb{P}_{\text{target}}(x_{t}, \theta, \lambda)\right) \end{aligned}
\end{equation}
where $Z_{s}$ and $Z_{t}$ are normalization constants, and $1-\lambda \sim \mathcal{U}([0, 1])$ defines the strength of the mixing, i.e. the size of the bounding box. The locations of the cutting and pasting regions are encoded as binary masks, i.e., $M_{s}, M_{t} \in \{0, 1\}^{H \times W}$, where a value of $1$ encodes for a patch in the cutting/pasting region. Under the above formalism, the mixing operation can be defined as:
\begin{equation}
\begin{aligned}
        x_{m} = (\textbf{1} - M_{t}) \odot x_{t} \\
        M_{t} \otimes x_{m} \leftarrow M_{s} \otimes x_{s} \\
        y_{m} = \lambda y_{t} + (1 - \lambda) y_{s}
\end{aligned}
\end{equation}
where $\textbf{1}$ is a mask of ones, $\odot$ denotes the element-wise multiplication, and $\otimes$ indicates an indexing w.r.t. a mask.
\vspace{1ex} \noindent \textbf{Computing the Semantic Distributions.}
Computing the semantic distributions of the target and source images is an essential part of the pipeline as it allows for a data-driven selection of the cutting/pasting sites, thereby avoiding the pitfalls of random selection. When the size of the bounding box matches that of a single patch, the distribution can be directly deduced from the self-attention map, as described in Sec.~\ref{subsec:method:TRoIs_model}.
As a consequence, and when the bounding box's size matches that of a single patch, the semantic distribution can be directly obtained from $\mathbb{P}_{\text{patch}}$ (see Eq.~\ref{eq:dist_patch}).
In practice, we would typically use bounding boxes encompassing more than a single patch. In that case, the distribution of the semantic content at the bounding box resolution can be obtained by a local aggregation of the distribution above:
\begin{equation}
\mathbb{P}_{\text{bbox}}(i) \propto \sum\nolimits_{j \in \mathcal{N}(i)}\mathbb{P}_{\text{patch}}(j)
\end{equation}
where $\mathcal{N}(i)$ returns the indices of the patches situated in the bounding box whose top left corner is the patch $i$. In practice, this can be efficiently implemented by first unflattening the patch distribution $\mathbb{P}_{\text{patch}}$, and convolving it with a kernel of ones and of the same dimension as the desired bounding box (see Fig.~\ref{fig:bbox_sampling}).


==> tables/bach_knn.tex <==
\begin{table}[ht]
\centering
\caption{\textbf{A weighted $k$ Nearest Neighbors classifier assesses the ability of the models to learn from uncurated data on the BACH dataset}. A 4-fold approach with $75\%/25\%$ train/test splits is used.}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{ l  c c c c c c}
\hline
       & \multicolumn{2}{c}{ScoreNet} & \multicolumn{2}{c}{TransPath \cite{wang2021transpath}} & \multicolumn{2}{c}{SwinTransformer \cite{liu2021swin}} \\
       \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
$k$ & Teacher & Student & Teacher & Student & Teacher & Student \\

\hline

\hline
\end{tabular}
}
\vspace{0.2cm}
\label{table:bach_knn}
\end{table}

